Less is More: Generating Grounded Navigation Instructions from Landmarks

We study the automatic generation of navigation instructions from 360-degree images captured on indoor routes. Existing generators suffer from poor visual grounding, causing them to rely on language priors and hallucinate objects. Our MARKY-MT5 system addresses this by focusing on visual landmarks; it comprises a first stage landmark detector and a second stage generator -- a multimodal, multilingual, multitask encoder-decoder. To train it, we bootstrap grounded landmark annotations on top of the Room-across-Room (RxR) dataset. Using text parsers, weak supervision from RxR's pose traces, and a multilingual image-text encoder trained on 1.8b images, we identify 971k English, Hindi and Telugu landmark descriptions and ground them to specific regions in panoramas. On Room-to-Room, human wayfinders obtain success rates (SR) of 71% following MARKY-MT5's instructions, just shy of their 75% SR following human instructions -- and well above SRs with other generators. Evaluations on RxR's longer, diverse paths obtain 61-64% SRs on three languages. Generating such high-quality navigation instructions in novel environments is a step towards conversational navigation tools and could facilitate larger-scale training of instruction-following agents.

==> notes_on_related_work.tex <==
\begin{itemize}
    \item Zhou et al. \cite{Yuanen-Zhou21}. They use a pre-trained text-image matcher to guide the model to learn keyword-bbox alignments, which is then used to condition their text generator.
    \begin{itemize}
        \item Similar: they also leverage text-bbox alignment;
        \item Different: a) different task: image captioning vs. navigation instruction generation; b) our edge in using MURAL-powered text-image encoder; c) our PMMX vs. their LSTM generator.
        
    \end{itemize}
    
    \item Huber et al. \cite{Huber18}. Image-grounded dialogue generation model that extracts sentiment information from images to imbue emotion into generated texts. Specialized datasets are used to train an image feature extractor to obtain sentiment features --- including scene understanding and sentiment, facial coding.
    \begin{itemize}
        \item Similar: image-grounded text generation that has a 2-stage component (i.e. rather than image->text direct generation, they mediate with specific image features for conditioning text generation).
        \item Different: a) last-gen architecture --- GRU + simple CNN vs. our SOTA/latest ones; b) dialogue vs. navigation, different challenges.
    \end{itemize}
    
    \item Wu et al. \cite{Qi-Wu22}. Introduing fine-grained, (sub-trajectory, sub-instruction) pairs for supervising navigation instruction generation. Other than the de-blackbox conditioning benefit that comes with a 2-stage image$\rightarrow$text generation process, they also use the pairs to ``reinitialize'' navigation agents during training such that it doesn't try to learn entire navigation paths in one-go but rather in small chunks.
    \begin{itemize}
        \item Similar: a) also in the navigation instruction generation domain; b) also uses an intermediate representation to bridge image$\rightarrow$text generation, in the form of sub-trajectories.
        \item Different: a) they don't create new instructions but rather squeeze out more supervision out of existing instructions with additional annotation; b) their definition of ``landmark'' differs from us: waypoints vs. our actual visual landmarks; c) their approach to augmentation is elicitation from human annotators while we have a more automatic/scalable design.
    \end{itemize}
    
    
    \item Jain and Sollami \cite{Jain21}. A language model with bimodal inputs: an image feature conditioner and a text encoder. Image and text features are extracted with independent encoders and they merged in a transformer decoder for text generation.
    \begin{itemize}
        \item Similar: image-grounded text generation.
        \item Different: a) theirs is not a 2-stage framework with an intermediate representation --- essentially still image$\rightarrow$text blackbox; b) general language modeling vs. navigation instruction generation.
    \end{itemize}
    
    
   \item Chan et al. \cite{EdgarChan12} present a survey of a wide range of studies showing the crucial role landmarks play in human navigation behavior.
    \begin{itemize} 
        \item ``Landmarks play an important role in guiding navigational behavior. A host of studies in the last 15 years has demonstrated that environmental objects can act as landmarks for navigation in different ways.''
        \item ``Visual information plays an important role in guiding navigation behaviors ... Individual differences in navigational abilities can also influence the type of landmark information that is encoded''
    \end{itemize}

    \item Foo et al. \cite{Foo05} found landmarks are the first means to depend on during navigation, and the perceptual channel of choice is visual.
    \begin{itemize} 
        \item ``Do humans integrate experience on specific routes into metric survey knowledge of the environment, or do they depend on a simpler strategy of landmark navigation? The authors tested this question using a novel shortcut paradigm during walking in a virtual environment. The authors find that participants could not take successful shortcuts in a desert world but could do so with dispersed landmarks in a forest ... depend on landmarks when they are available.''
        \item ``... Visual is the most important channel for landmarking: “... the use of visual information appears to be predominant ...''
    \end{itemize}
    
    \item Epistein and Vass \cite{Epstein14} investigate the role of landmark-based navigation from the biological/neurological angle and demonstrate how the behavior is wired and specialized in human brain (related, Marchette et al. \cite{Marchette15} look at how landmarking is generalized and ``encoded''  in human brain).
    \begin{itemize}  
        \item ``Humans and animals use landmarks during wayfinding to determine their position and heading. This strategy, known as landmark-based piloting ...''
        \item ``This evidence suggests that the parahippocampal place area is critical for landmark recognition ...''
    \end{itemize}
    
    \item Yesiltepe et al. \cite{Yesiltepe21} review the psychology literature to how landmarks are utilized in human navigation. Classifying different types of landmarks and study the concept of saliency in landmarking.

    
\end{itemize}
